TAG: Learning Circuit Spatial Embedding From Layouts

Analog and mixed-signal (AMS) circuit designs still rely on human design expertise. Machine learning has been assisting circuit design automation by replacing human experience with artificial intelligence. This paper presents TAG, a new paradigm of learning the circuit representation from layouts leveraging text, self-attention and graph. The embedding network model learns spatial information without manual labeling. We introduce text embedding and a self-attention mechanism to AMS circuit learning. Experimental results demonstrate the ability to predict layout distances between instances with industrial FinFET technology benchmarks. The effectiveness of the circuit representation is verified by showing the transferability to three other learning tasks with limited data in the case studies: layout matching prediction, wirelength estimation, and net parasitic capacitance prediction.

==> texlib/ieee_setting.tex <==
% =============================================================
%            setting for IEEE format paper
%
%   Author      : Bei Yu
%   Last Update : 06/2015
% =============================================================


\usepackage[noend]{algpseudocode}
%\usepackage{algpseudocode}    % new algorithm package
\usepackage{algorithm}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{amsfonts}
\usepackage{booktabs}
\usepackage{multirow}
\usepackage{graphicx}         % include pdf figures
\usepackage{color}
\usepackage{cite}             % more citations in one bracket
\usepackage{comment}          % use comment
\usepackage{soul}             % use highlight command \hl{}
\soulregister\cite7
\soulregister\ref7
\soulregister\pageref7
\usepackage{amsthm}
\usepackage{etoolbox}         % commands \newtoggle, \toggletrue, \iftoggle
\usepackage{url}
\usepackage{nth}              % nth command
\usepackage{bm}               % bm command
\usepackage{caption} 
\usepackage{subfig}

\usepackage{cleveref}                                      % smart



\newtheorem{myproblem}{\textbf{Problem}}
\newtheorem{mydefinition}{\textbf{Definition}}
\newtheorem{mytheorem}{\textbf{Theorem}}
\newtheorem{mylemma}{\textbf{Lemma}}
\newtheorem{myclaim}{\textbf{Claim}}
\newtheorem{myapplication}{\textbf{Application}}
\newtheorem{myconjecture}{Conjecture}

% ==== Local new commands
%\newcommand{\calH}{\mathcal{H}}
%\newcommand{\calN}{\mathcal{N}}
\newcommand{\calO}{\mathcal{O}}
%\newcommand{\calP}{\mathcal{P}}
%\newcommand{\calV}{\mathcal{V}}
%\newcommand{\calS}{\mathcal{S}}
%\newcommand{\calD}{\mathcal{D}}
\newcommand{\norm}[1]{\left\lVert#1\right\rVert}
\renewcommand{\vec}[1]{\boldsymbol{#1}} 
%\newcommand{\m}[1]{\mathbf{#1}}
%\newcommand{\mx}{\m{x}}
%\newcommand{\my}{\m{y}}
%\newcommand{\mz}{\m{z}}
\DeclareMathOperator*{\argmin}{argmin}

% long line in algorithm
% e.g.: \Statex[4] ...;
\makeatletter
\let\OldStatex\Statex
\renewcommand{\Statex}[1][3]{%
  \setlength\@tempdima{\algorithmicindent}%
  \OldStatex\hskip\dimexpr#1\@tempdima\relax
}
\makeatother


% ==== Logs:
%
%  06/2015: clean IEEEtranBSTCTL commands
%  11/2014: \solregister, to support highlight to mybox, definition, and citations
%  10/2014: add package "authblk" & "bm"
%  09/2014: "problem" => "myproblem"
%  07/2014: introduce \Statex[] for lone algorithmic statement
%  05/2014: new package {soul} to use highlight command \hl{}
%




==> texlib/poster_setting.tex <==
% ============================================================
%             Beamer poster setting file
%
%   Author      : Bei Yu
%   last Update : 06/2014
% ============================================================

% additional settings
\setbeamerfont{itemize}{size=\normalsize}
\setbeamerfont{itemize/enumerate body}{size=\normalsize}
\setbeamerfont{itemize/enumerate subbody}{size=\normalsize}


% block width setting
\newenvironment<>{varblock}[2][\textwidth]{%
  \setlength{\textwidth}{#1}
  \setbeamercolor{block title}{fg=white,bg=blue!20!green}
  %\setbeamercolor{block body}{fg=black,bg=olive!50}
  \setbeamercolor{block body}{fg=black,bg=blue!10}
  \begin{actionenv}#3%
  \def\insertblocktitle{#2}%
  \par%
  \usebeamertemplate{block begin}}
  {
    \par%
    \usebeamertemplate{block end}%
    \end{actionenv}
  }


% abbreviations
\usepackage{xspace}
\makeatletter
\DeclareRobustCommand\onedot{\futurelet\@let@token\@onedot}
\def\@onedot{\ifx\@let@token.\else.\null\fi\xspace}
\def\eg{{e.g}\onedot} \def\Eg{{E.g}\onedot}
\def\ie{{i.e}\onedot} \def\Ie{{I.e}\onedot}
\def\cf{{c.f}\onedot} \def\Cf{{C.f}\onedot}
\def\etc{{etc}\onedot}
\def\vs{{vs}\onedot}
\def\wrt{w.r.t\onedot}
\def\dof{d.o.f\onedot}
\def\etal{{et al}\onedot}
\makeatother


% === including packages
\usepackage{bm}
\usepackage{xcolor}
\usepackage{colortbl}
\usepackage{times}
\usepackage{amsmath,amsthm, amssymb, latexsym}
\usepackage{exscale}
\usepackage{subfigure}
\usepackage{multirow}
\usepackage{comment}
\usepackage{booktabs, array}
\usepackage[english]{babel}
\usepackage[latin1]{inputenc}
\usepackage[orientation=landscape,size=custom,width=200,height=230,scale=1.9]{beamerposter}
\listfiles

% =====  algorithm setting
%\usepackage[noend]{algpseudocode}
\usepackage{algpseudocode}
\usepackage{algorithm}
%\renewcommand{\algorithmicrequire}{\textbf{Input:}}  % Use Input in the format of Algorithm
%\renewcommand{\algorithmicensure}{\textbf{Output:}} % Use Output in the format of Algorithm

% ==== Log
%
%  05/2014: preliminary results show that pgf library is NOT good for poster
%


